Building Multi-Agent Copilot towards Autonomous Agricultural Data Management and Analysis

Current agricultural data management and analysis paradigms are to large extent traditional, in which data collecting, curating, integration, loading, storing, sharing and analyzing still involve too much human effort and know-how. The experts, researchers and the farm operators need to understand the data and the whole process of data management pipeline to make fully use of the data. The essential problem of the traditional paradigm is the lack of a layer of orchestrational intelligence which can understand, organize and coordinate the data processing utilities to maximize data management and analysis outcome. The emerging reasoning and tool mastering abilities of large language models (LLM) make it a potentially good fit to this position, which helps a shift from the traditional user-driven paradigm to AI-driven paradigm. In this paper, we propose and explore the idea of a LLM based copilot for autonomous agricultural data management and analysis. Based on our previously developed platform of Agricultural Data Management and Analytics (ADMA), we build a proof-of-concept multi-agent system called ADMA Copilot, which can understand user's intent, makes plans for data processing pipeline and accomplishes tasks automatically, in which three agents: a LLM based controller, an input formatter and an output formatter collaborate together. Different from existing LLM based solutions, by defining a meta-program graph, our work decouples control flow and data flow to enhance the predictability of the behaviour of the agents. Experiments demonstrates the intelligence, autonomy, efficacy, efficiency, extensibility, flexibility and privacy of our system. Comparison is also made between ours and existing systems to show the superiority and potential of our system.

==> sec_implementation.tex <==
\section{Implementation}
\label{sec:implementation}

Based on the design ideology and framework proposed in Section \ref{sec:design}, we introduce the ADMA implementation in detail.

\subsection{System Components}

ADMA contains seven components: data source, batch processing, real-time processing, actuators, server, front end and JupyterHub. Figure~\ref{fig:components} illustrates the architectures of the six components.




The data source can be further categorized into 5 classes: database for storing raw data, file system for storing raw data, sensors for collecting real-time data ,database for storing metadata and vector database for storing high dimensional vector representations of data.

The batch processing component is the engine of the whole system. The containerized environment can host various types of containerized tools such as R, Python, Matlab, Tensorflow, Cuda, MPI, and many more customized tools for the specific disciplines. There is a  container scheduler such as Swarm or Kubernetes to manage the running of containers. Various user-defined data processing and model training can be conducted in the container environment. The output of the batch processing will be stored back to the data source for further retrieval and processing.

The real-time processing component connects to the sensors and uses pipes to stream the real-time data for further processing. Similar to batch processing, a containerized environment is also supported, where hosted pre-trained models and customized tools can process data and make decisions in a real-time or near real-time fashion.  The real-time analytical results can be fed to the data processing module and data service API inside the server component. The decisions and commands can be output to the actuator to execute. This component is a necessary complement to batch processing when real-time analysis and control are required, and relatively low accuracy is tolerated.

The actuator is included in the system to make it more like a fully functioning control system. Connected to the real-time processing component, the actuator executes the commands/decisions output by the hosted models or user-coded tools. The types of actuators vary among different disciplines. For biological system engineering, to name a few, there are actuators such as irrigation systems, robotics, and field operation machines. 

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pics/search_1_cr.png}
        \caption{Search Box}
        \label{fig:data_search_1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pics/search_2_cr.png}
        \caption{Map Visualization}
        \label{fig:data_search_2}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pics/search_3_cr.png}
        \caption{Embedding Visualization}
        \label{fig:data_search_3}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pics/search_4_cr.png}
        \caption{Search Results List}
        \label{fig:data_search_4}
    \end{subfigure}%
    \hfill   

    \caption{Data Search}
    \label{fig:data_search}
\end{figure}

The server is the operational handler of the whole system. The data management module is responsible for ordinary operations such as file search, retrieve, upload, delete, update, and processing. The tool management module keeps the information of the tool sets used in the system. The model management module is responsible for maintaining all the pre-trained models. The data processing module talks to and manages the batch processing and real-time processing components. This module is an umbrella module for all the data processing jobs, such as data pre-processing, data co-locating, batch processing, model training,  model hosting, real-time processing, etc. The security and authentication module guarantees the data storage and transmission is secure, and each user has separate access permission and view of the data. Data service API acts as the portal for the front end to manipulate the data in our system.  



The front end runs on the user-side machine and can be a web browser, command-line, or third-party software. The front end communicates with the server through the data service API. Users of our system can conduct ordinary file management operations and initiate data processing requests to the system. The analytical results can be displayed in the front end for the user to view.

To provide the users with more flexibility, ADMA connects with JupyterHub. Each user can create their own JupyterLab, which is the latest web-based interactive development environment for notebooks, code, and data in the field of data science, scientific computing, computational journalism, and machine learning. User can utilize the same workspace to put their data and tools in both ADMA and JupyterLab, in this way the user can shift between two systems seamlessly. 



%\subsection{System Deployment}




